Challenges and Pitfalls of Machine Learning Evaluation and Benchmarking

An increasingly complex and diverse collection of Machine Learning (ML) models as well as hardware/software stacks, collectively referred to as "ML artifacts", are being proposed - leading to a diverse landscape of ML. These ML innovations proposed have outpaced researchers' ability to analyze, study and adapt them. This is exacerbated by the complicated and sometimes non-reproducible procedures for ML evaluation. A common practice of sharing ML artifacts is through repositories where artifact authors post ad-hoc code and some documentation, but often fail to reveal critical information for others to reproduce their results. This results in users' inability to compare with artifact authors' claims or adapt the model to his/her own use. This paper discusses common challenges and pitfalls of ML evaluation and benchmarking, which can be used as a guideline for ML model authors when sharing ML artifacts, and for system developers when benchmarking or designing ML systems.

==> latex_tools/comment.tex <==


\definecolor{oldeditorcolor}{rgb}{0.215686,0.494118,0.721569}

% Select what to do with command \comment:
% \newcommand{\comment}[1]{}  %comment not showed
% \newcommand{\comment}[1]{\todo[inline]{\bfseries \color{blue} #1 }} %comment showed

\newif\ifsubmit
\submittrue
% \submitfalse
\ifsubmit
    \usepackage[disable]{todonotes} % notes not showed
    \newcommand{\usure}[1]{}
    \newcommand{\change}[1]{}
    \newcommand{\info}[1]{}
    \newcommand{\improvement}[1]{}
    \newcommandx{\cheng}[2][1=]{}
    \newcommandx{\abdul}[2][1=]{}
    \newcommandx{\abi}[2][1=]{}
    \newcommandx{\renee}[2][1=]{}
    \newcommandx{\junjun}[2][1=]{}
    \newcommandx{\wenmei}[2][1=]{}
    \newcommandx{\old}[2][1=]{}
    \newcommandx{\delete}[2][1=]{}
\else
\usepackage[
    colorinlistoftodos,
    prependcaption,
    draft,
    textsize=tiny,
    obeyFinal,
    textwidth=2cm
]{todonotes}
% 	\usepackage{geometry}
% 	\reversemarginpar
	\newcounter{todocounter} 
	\newcounter{adtodocounter} 
	\newcounter{cltodocounter} 
	\newcounter{jjtodocounter} 
	\newcounter{wmhtodocounter} 
	\newcounter{abtodocounter} 
	\newcounter{rntodocounter} 
	\newcounter{oldtodocounter} 
	\newcounter{deletetodocounter} 
    \newcommandx{\unsure}[2][1=]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
    \newcommandx{\change}[2][1=]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
    \newcommandx{\info}[2][1=]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,#1]{#2}}
    \newcommandx{\improvement}[2][1=]{ \marginpar[\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{#2}]{}}
    \newcommandx{\thiswillnotshow}[2][1=]{\todo[disable,#1]{#2}}
    \newcommandx{\cheng}[2][1=]{\stepcounter{cltodocounter} \todo[linecolor=red,backgroundcolor=purple!25,bordercolor=purple,#1]{CL(\thecltodocounter): #2}}
    \newcommandx{\abdul}[2][1=]{\stepcounter{adtodocounter} \todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{AD(\theadtodocounter): #2}}
    \newcommandx{\abi}[2][1=]{\stepcounter{abtodocounter} \todo[linecolor=teal,backgroundcolor=teal!25,bordercolor=teal,#1]{AB(\theabtodocounter): #2}}
    \newcommandx{\renee}[2][1=]{\stepcounter{rntodocounter} \todo[linecolor=yellow,backgroundcolor=yello!25,bordercolor=OliveGreen,#1]{RN(\therntodocounter): #2}}
    \newcommandx{\jinjun}[2][1=]{\stepcounter{jjtodocounter} \todo[linecolor=yellow,backgroundcolor=yellow!25,bordercolor=yellow,#1]{JJ(\thejjtodocounter): #2}}
    \newcommandx{\wenmei}[2][1=]{\stepcounter{wmhtodocounter} \todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,#1]{WH(\thewmhtodocounter): #2}}
    \newcommandx{\old}[2][1=]{\stepcounter{oldtodocounter} \todo[linecolor=oldeditorcolor,backgroundcolor=oldeditorcolor!25,bordercolor=oldeditorcolor,#1]{OLD(\theoldtodocounter): #2}}
    \newcommandx{\delete}[2][1=]{\stepcounter{deletetodocounter} \todo[linecolor=oldeditorcolor,backgroundcolor=oldeditorcolor!25,bordercolor=oldeditorcolor,#1]{OLD(\thedeletetodocounter): #2}}
\fi

==> latex_tools/lstcpp.tex <==

\usepackage{listings}



\definecolor{myred}{rgb}{0.843137,0.188235,0.152941}
\definecolor{myblack}{rgb}{0.27451,0.32549,0.384314}
\definecolor{mygreen}{rgb}{0.301961,0.686275,0.290196}
\definecolor{myyellow}{rgb}{0.996078,0.878431,0.564706}
\definecolor{myblue}{rgb}{0.568627,0.74902,0.858824}


\lstset{
  frame=single,
  language=C++,
  tabsize=1,
  title=\lstname,
  basicstyle=\small\ttfamily,
  keywordstyle=\color{myblack}\ttfamily,
  stringstyle=\color{myred}\ttfamily,
  commentstyle=\color{mygreen}\ttfamily
}




==> latex_tools/protobuf.tex <==

\definecolor{pbgray}{rgb}{0.5,0.5,0.5}
\lstdefinelanguage[2]{protobuf}{%
    sensitive=true,%
    numbers=left,
	breaklines=true,
    mathescape=true,
    xleftmargin=2em,
    framexleftmargin=3em,
    stepnumber=1,
    escapechar=|,
    numberstyle=\tiny\color{pbgray},  
    frame=single,
    morecomment=[l]{//},%
    morestring=[b]{"},%
    % For the keywords of Protocol Buffers
    % see https://developers.google.com/protocol-buffers/docs/proto
    morekeywords={enum,oneof,map,syntax,public,import,option,package,message,%
        group,optional,required,repeated,default,reserved,extend,extensions,%
        to,max,service,rpc,returns,true,false},%
    % Basic types
    % see https://developers.google.com/protocol-buffers/docs/proto#scalar
    morekeywords=[2]{%
        double,float,int32,int64,uint32,uint64,sint32,sint64,%
        fixed32,fixed64,sfixed32,sfixed64,bool,string,bytes},%
    % Options
    % taken from 'google/protobuf/descriptor.proto'
    morekeywords=[3]{%
        % Generic Options
        deprecated, uninterpreted_option,%
        % File Options
        java_package,java_outer_classname,java_multiple_files,%
        java_generate_equals_and_hash,java_string_check_utf8,optimize_for,%
        go_package,cc_generic_services,java_generic_services,%
        py_generic_services,cc_enable_arenas,obj_class_prefix,%
        csharp_namespace,%
        % Message Options
        message_set_wire_format,no_standard_descriptor_accessor,map_entry,%
        % Field Options
        ctype, packed,jstype,lazy,weak,%
        % Enum Options
        allow_alias}%
}
\lstalias[]{protobuf2}[2]{protobuf}

\lstdefinelanguage[3]{protobuf}[2]{protobuf}{%
    % Language keywords
    % see https://developers.google.com/protocol-buffers/docs/proto3
    deletekeywords={
        % 'group' was marked as deprecated in protobuf2; now it's disallowed
        group,%
        % in protobuf3 the Any type replaces extensions (from protobuf2)
        extensions, to, extend, max,%
        % 'required' is no longer allowed
        required,%
        % 'optional' is default; stating it explicitly is disallowed
        optional,%
        % explicit default values are no longer allowed
        default}%
}
\lstalias[]{protobuf3}[3]{protobuf}

==> latex_tools/protobuf_style.tex <==
\usepackage{xcolor}
\usepackage{xcolor-solarized}
\usepackage{textcomp}

\newcommand{\SetProtoColorsSolarized}{
  % Colors taken from the 'solarized' color scheme of Ethan Schoonover
  % (with light background)
  % http://ethanschoonover.com/solarized
  \colorlet{proto_basic}{solarized-base00}
  \colorlet{proto_keyword}{solarized-cyan}
  \colorlet{proto_type}{solarized-cyan}
  \colorlet{proto_options}{solarized-cyan}
  \colorlet{proto_comment}{solarized-base1}
  \colorlet{proto_string}{solarized-blue}
  \colorlet{proto_number}{solarized-violet}
  \colorlet{proto_ident}{solarized-base00}
  \colorlet{proto_digits}{solarized-violet}
  \colorlet{proto_background}{solarized-base3}
}

\newcommand{\SetProtoColorsBlueish}{
  % Colors inspired by the NASM style of Robin Eklind
  % https://github.com/mewspring/latex
  \definecolor{proto_basic}{RGB}{0,0,0}             % black
  \definecolor{proto_keyword}{RGB}{0,0,255}         % blue
  \definecolor{proto_type}{RGB}{128,0,0}            % dark red
  \definecolor{proto_options}{RGB}{128,0,128}       % purple
  \definecolor{proto_comment}{RGB}{0,128,0}         % dark green
  \definecolor{proto_string}{RGB}{255,0,0}          % red
  \definecolor{proto_number}{RGB}{108,113,196}      % violet
  \definecolor{proto_ident}{RGB}{0,0,0}             % black
  \definecolor{proto_digits}{RGB}{0,0,128}          % dark blue
  \definecolor{proto_background}{RGB}{255,255,255}  % white
}

\newcommand{\SetProtoColorsTomorrow}{
  % Colors taken from the 'Tomorrow' color scheme of Chris Kempson
  % https://github.com/chriskempson/tomorrow-theme/blob/master/vim/colors/Tomorrow.vim
  \definecolor{proto_basic}{RGB}{0, 0, 0}          % dark grey
  \definecolor{proto_keyword}{RGB}{0,0,0}      % orange
  \definecolor{proto_type}{RGB}{255,0,0}        % purple
  \definecolor{proto_options}{RGB}{0, 0, 0}
  \definecolor{proto_comment}{RGB}{142, 144, 140}
  \definecolor{proto_string}{RGB}{0, 0, 0}        % green
  \definecolor{proto_number}{RGB}{0,0,0}
  \definecolor{proto_ident}{RGB}{0,0,255}         % red
  \definecolor{proto_digits}{RGB}{0,0,255}       % orange
  \definecolor{proto_background}{RGB}{255, 255, 255}  % white
}


% \SetProtoColorsSolarized{}
\SetProtoColorsTomorrow{}
%\SetProtoColorsBlueish{}



\lstdefinestyle{protobuf}{
%   frame=lines,
    % captionpos=b,
  backgroundcolor=\color{proto_background},
  basicstyle=\color{proto_basic}\fontsize{7}{7}\ttfamily,
	keywordstyle=[1]\fontsize{7}{7}\ttfamily\mdseries\color{proto_keyword},
	keywordstyle=[2]\fontsize{7}{7}\ttfamily\mdseries\color{proto_type},
	keywordstyle=[3]\fontsize{7}{7}\ttfamily\mdseries\color{proto_options},
	commentstyle= \fontsize{7}{7}\color{purple}\ttfamily\fontsize{7}{7}\ttfamily,
	stringstyle=\color{proto_string},
  identifierstyle=\color{proto_ident},
	breaklines=true,
	showstringspaces=false,
	tabsize=2,
  % This 'literate' block is responsible for colouring numbers
  % appearing in the code
  literate={0}{{\textcolor{proto_digits}{0}}}{1}%
           {1}{{\textcolor{proto_digits}{1}}}{1}%
           {2}{{\textcolor{proto_digits}{2}}}{1}%
           {3}{{\textcolor{proto_digits}{3}}}{1}%
           {4}{{\textcolor{proto_digits}{4}}}{1}%
           {5}{{\textcolor{proto_digits}{5}}}{1}%
           {6}{{\textcolor{proto_digits}{6}}}{1}%
           {7}{{\textcolor{proto_digits}{7}}}{1}%
           {8}{{\textcolor{proto_digits}{8}}}{1}%
           {9}{{\textcolor{proto_digits}{9}}}{1}%
           {.0}{{\textcolor{proto_digits}{.0}}}{2}%
           {.1}{{\textcolor{proto_digits}{.1}}}{2}%
           {.2}{{\textcolor{proto_digits}{.2}}}{2}%
           {.3}{{\textcolor{proto_digits}{.3}}}{2}%
           {.4}{{\textcolor{proto_digits}{.4}}}{2}%
           {.5}{{\textcolor{proto_digits}{.5}}}{2}%
           {.6}{{\textcolor{proto_digits}{.6}}}{2}%
           {.7}{{\textcolor{proto_digits}{.7}}}{2}%
           {.8}{{\textcolor{proto_digits}{.8}}}{2}%
           {.9}{{\textcolor{proto_digits}{.9}}}{2}%
           % We need to add some hacks - otherwise 'listings' would
           % colour (only) the digits in the types instead of the type
           {int32}{{\textcolor{proto_type}{int32}}}{5}%
           {int64}{{\textcolor{proto_type}{int64}}}{5}%
           {uint32}{{\textcolor{proto_type}{uint32}}}{6}%
           {uint64}{{\textcolor{proto_type}{uint64}}}{6}%
           {sint32}{{\textcolor{proto_type}{sint32}}}{6}%
           {sint64}{{\textcolor{proto_type}{sint64}}}{6}%
           {fixed32}{{\textcolor{proto_type}{fixed32}}}{7}%
           {fixed64}{{\textcolor{proto_type}{fixed64}}}{7}%
           {sfixed32}{{\textcolor{proto_type}{sfixed32}}}{8}%
           {sfixed64}{{\textcolor{proto_type}{sfixed64}}}{8}%
           {java_string_check_utf8}{{%
             \textcolor{proto_options}{java_string_check_utf8}}}{2}%
           {\ }{{ }}{1},
	prebreak=\raisebox{0ex}[0ex][0ex]{\ensuremath{\hookleftarrow}},
	upquote=true,
}

==> latex_tools/yaml.tex <==
\definecolor{yamlred}{rgb}{0.843137,0.188235,0.152941}
\definecolor{yamlblue}{rgb}{0.27451,0.32549,0.384314}
\definecolor{yamlkey}{rgb}{0.980392,0.501961,0.447059}

\newcommand\YAMLfontsize{\fontsize{7}{7}}
\newcommand\YAMLcolonstyle{\color{black}\mdseries\YAMLfontsize\ttfamily}
\newcommand\YAMLkeystyle{\bfseries\color{yamlblue}\YAMLfontsize\ttfamily}
\newcommand\YAMLvaluestyle{\color{black}\mdseries\YAMLfontsize\ttfamily}



% here is a macro expanding to the name of the language
% (handy if you decide to change it further down the road)

\definecolor{yamlgray}{rgb}{0.5,0.5,0.5}
\lstdefinelanguage{yaml}
{
  keywords={true,false,null,y,n},
  keywordstyle=\YAMLvaluestyle,
  basicstyle=\YAMLfontsize\YAMLkeystyle,                                 % assuming a key comes first
  sensitive=false,
  comment=[l]{\#},
  morecomment=[s]{/*}{*/},
  commentstyle=\YAMLcolonstyle\color{yamlred}\ttfamily\YAMLfontsize\ttfamily,
  stringstyle=\YAMLvaluestyle\ttfamily\YAMLfontsize\ttfamily,
  moredelim=[l][\color{orange}]{\&},
  moredelim=[l][\color{yamlred}]{*},
  moredelim=**[il][\YAMLcolonstyle{:}\YAMLvaluestyle]{:},   % switch to value style at :
  morestring=[b]',
  morestring=[b]",
  literate =    {---}{{\ProcessThreeDashes}}3
                {>}{{\textcolor{yamlred}\textbar}}1     
                {|}{{\textcolor{yamlred}\textbar}}1 
                {\ -\ }{{\mdseries\ -\ }}3,       
    % frame=single,
    frame=top,
    frame=bottom,
    numbers=left,
    % framerule=1pt,
    rulesep=1pt,
	breaklines=true,
    mathescape=true,
    xleftmargin=2em,
    framexleftmargin=3em,
    stepnumber=1,
    escapechar=|,
    captionpos=t,
    numberstyle=\tiny\color{yamlgray},
}

% switch to key style at EOL
% \lst@AddToHook{EveryLine}{\ifx\lst@language yaml\YAMLkeystyle\fi}
\makeatother

\newcommand\ProcessThreeDashes{\llap{\color{cyan}\mdseries-{-}-}}

